Obstacle Identification and Ellipsoidal Decomposition for Fast Motion Planning in Unknown Dynamic Environments

Collision avoidance in the presence of dynamic obstacles in unknown environments is one of the most critical challenges for unmanned systems. In this paper, we present a method that identifies obstacles in terms of ellipsoids to estimate linear and angular obstacle velocities. Our proposed method is based on the idea of any object can be approximately expressed by ellipsoids. To achieve this, we propose a method based on variational Bayesian estimation of Gaussian mixture model, the Kyachiyan algorithm, and a refinement algorithm. Our proposed method does not require knowledge of the number of clusters and can operate in real-time, unlike existing optimization-based methods. In addition, we define an ellipsoid-based feature vector to match obstacles given two timely close point frames. Our method can be applied to any environment with static and dynamic obstacles, including the ones with rotating obstacles. We compare our algorithm with other clustering methods and show that when coupled with a trajectory planner, the overall system can efficiently traverse unknown environments in the presence of dynamic obstacles.

==> macros.tex <==
\newcommand{\myred}{red!15}
\newcommand{\mygreen}{green!15}
\newcommand{\myorange}{orange!15}
\newcommand{\myblue}{blue!15}

\newcommand{\vect}[3]{{_{\mathsmaller{\mathrm{#2}}}\mathbf{#1}_{\mathsmaller{\mathrm{#3}}}}} %
\newcommand{\wfr}[0]{\ensuremath{\mathcal{W}}} %
\newcommand{\bfr}[0]{\ensuremath{\mathcal{B}}} %
\newcommand{\cfr}[0]{\ensuremath{\mathcal{C}}} %
\newcommand{\pfr}[0]{\ensuremath{\mathcal{P}}}
\newcommand{\heading}[0]{\psi}

\newcommand{\rotateRPY}[3]%
{   \pgfmathsetmacro{\rollangle}{#1}
    \pgfmathsetmacro{\pitchangle}{#2}
    \pgfmathsetmacro{\yawangle}{#3}

    \pgfmathsetmacro{\newxx}{cos(\yawangle)*cos(\pitchangle)}
    \pgfmathsetmacro{\newxy}{sin(\yawangle)*cos(\pitchangle)}
    \pgfmathsetmacro{\newxz}{-sin(\pitchangle)}
    \path (\newxx,\newxy,\newxz);
    \pgfgetlastxy{\nxx}{\nxy};

    \pgfmathsetmacro{\newyx}{cos(\yawangle)*sin(\pitchangle)*sin(\rollangle)-sin(\yawangle)*cos(\rollangle)}
    \pgfmathsetmacro{\newyy}{sin(\yawangle)*sin(\pitchangle)*sin(\rollangle)+ cos(\yawangle)*cos(\rollangle)}
    \pgfmathsetmacro{\newyz}{cos(\pitchangle)*sin(\rollangle)}
    \path (\newyx,\newyy,\newyz);
    \pgfgetlastxy{\nyx}{\nyy};

    \pgfmathsetmacro{\newzx}{cos(\yawangle)*sin(\pitchangle)*cos(\rollangle)+ sin(\yawangle)*sin(\rollangle)}
    \pgfmathsetmacro{\newzy}{sin(\yawangle)*sin(\pitchangle)*cos(\rollangle)-cos(\yawangle)*sin(\rollangle)}
    \pgfmathsetmacro{\newzz}{cos(\pitchangle)*cos(\rollangle)}
    \path (\newzx,\newzy,\newzz);
    \pgfgetlastxy{\nzx}{\nzy};
}

\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcommand\setrow[1]{\gdef\rowmac{#1}#1\ignorespaces}
\newcommand\clearrow{\global\let\rowmac\relax}
\clearrow

\newcommand{\pos}{\text{pos}}
\newcommand{\att}{\text{att}}
\newcommand{\cmd}{\text{cmd}}
\newcommand{\err}{\text{err}}
\newcommand{\des}{\text{ref}}
\renewcommand{\i}{\text{i}}

\newcommand{\diff}[2]{\frac{\delta #1}{\delta #2}}
\newcommand{\mat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\renewcommand{\skew}[1]{\lbrack\bm{#1}\rbrack_{\!\times}}

\newcommand{\rom}[1]{\expandafter{\romannumeral #1\relax}}
\newcommand{\qmarks}[1]{``#1"}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\hide}[1]{}
\newcommand{\davide}[1]{{\color{red} Davide: #1}}
\newcommand{\elia}[1]{{\color{olive} Elia: #1}}
\newcommand{\TODO}[1]{{\color{blue} TODO: #1}}
\newcommand{\rev}[1]{{\color{black}#1}}
\newcommand\icra[1]{\textcolor{black}{#1}}


\definecolor{c1}{HTML}{D9B08C}
\definecolor{c2}{HTML}{FFCB9A}
\definecolor{c3}{HTML}{D1E8FF}
\definecolor{c4}{HTML}{DEF2F1}

